Relativistic Monte Carlo

Hamiltonian Monte Carlo (HMC) is a popular Markov chain Monte Carlo (MCMC) algorithm that generates proposals for a Metropolis-Hastings algorithm by simulating the dynamics of a Hamiltonian system. However, HMC is sensitive to large time discretizations and performs poorly if there is a mismatch between the spatial geometry of the target distribution and the scales of the momentum distribution. In particular the mass matrix of HMC is hard to tune well. In order to alleviate these problems we propose relativistic Hamiltonian Monte Carlo, a version of HMC based on relativistic dynamics that introduce a maximum velocity on particles. We also derive stochastic gradient versions of the algorithm and show that the resulting algorithms bear interesting relationships to gradient clipping, RMSprop, Adagrad and Adam, popular optimisation methods in deep learning. Based on this, we develop relativistic stochastic gradient descent by taking the zero-temperature limit of relativistic stochastic gradient Hamiltonian Monte Carlo. In experiments we show that the relativistic algorithms perform better than classical Newtonian variants and Adam.

==> GMM.tex <==
We considered a simple univariate model obtained by combining the three following Gaussian random variables with equal mixing proportions: $ \mathcal{N}(-5,1/ \sigma^2)$,  $\mathcal{N}(0,\sigma^2)$,  $\mathcal{N}(5,1/\sigma^2)$. We picked the value of $\sigma^2$ from the set $\{1,0.5,0.3 \}$, giving rise to three different Gaussian mixture models (plotted in the top row of Figure \ref{fig:GMM}). Note that when $\sigma^2=1$ the three Gaussians have the same variance and, the lower $\sigma^2$, the larger the discrepancy between their variances and thus the wider the range of values taken by the gradient of the model. We compared the performance of NHMC and RHMC for a wide range of stepsize values. The goal was to verify whether the relativistic dynamics is more robust to the choice of the stepsize and allows for a more efficient exploration of the target density.  


Figure \ref{fig:GMM} shows the mean absolute error (MAE), the log Stein discrepancy and the effective sample size (ESS) as a function of the stepsize for each of the three Gaussian mixture models. The MAE is computed as the L1 distance between the sample frequencies and the true probabilities, obtained by partitioning the interval [-10,10] with 100 bins of size 0.2. The Stein discrepancy is a measure to quantify the maximum discrepancy between sample and target expectations \citep{Stein2015}. The MAE and Stein discrepancy were averaged over 100 chains each with $1 \times 10^6$ samples. In the examples in this section, we set the mass parameter $m=1$ and the number of leapfrog steps to 10 in both RHMC and NHMC and $c=1$ in RHMC. RHMC shows to be strikingly more robust to the stepsize compared to NHMC, which fails to explore the target distribution and results in a large MAE and log stein discrepancy, especially when the stepsize is large. Moreover, when the gradients of the target model span a large range of values, the improvements yielded by the relativistic dynamics are more pronounced. These results confirm that, since the speed of particles is bounded by $c$, RHMC is less sensitive to the presence of peaked gradients in the target density and more stable with respect to the choice of the stepsize. 

 Moreover, RHMC reaches larger ESS values and therefore is able to explore the target density more efficiently than NHMC for a wide range of stepsizes.

Finally, we picked the optimal step sizes minimising the MAE error and compared the ESS of the Markov chains for the two algorithms. The ESS values at the optimal stepsize are shown in Table \ref{table:ESS}, where we report the mean and one standard deviation after running 100 different chains of $1 \times 10^6$ samples each. RHMC consistently outperforms NHMC and, as expected, this improvement is particularly pronounced in Model 3, where the gradient of the target model spans a large range of values. 


\begin{figure*}[]
\centering


\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/model1}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/model05}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/model03}
\end{subfigure}

\vspace{-0.5cm}

\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/MAE1}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/MAE05}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/MAE03}
\end{subfigure}

\vspace{-0.5cm}

\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/STEIN1}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/STEIN05}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/STEIN03}
\end{subfigure}

\vspace{-0.5cm}

\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/ESS1}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/ESS05}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\centering
\includegraphics[width=\columnwidth]{plots_GMM/ESS03}
\end{subfigure}


\caption{Mean absolute error (MAE), log Stein discrepancy and effective sample size (ESS) against stepsize for three different Gaussian mixture models.}
\label{fig:GMM}
\end{figure*}


\begin{table}[]
\centering
\caption{Comparison of the ESS for RHMC and NHMC given the optimal stepsize minimizing the MAE. The table reports the mean ESS and one standard deviation over 100 different runs.}
\label{table:ESS}
\begin{tabular}{|l|l|l|l|l|}
\hline
ESS  & Model 1 & Model 2 & Model 3 \\ \hline
RHMC &\textbf{70119.5}  $\pm$ \textbf{875.3}  & \textbf{47785.0} $\pm$ \textbf{848.0} & \textbf{109659.9}  $\pm$ \textbf{1408.8}   \\ \hline

NHMC &35970.8  $\pm$ 558.5 &29659.6  $\pm$   577.1  &  20675.4 $\pm$ 558.5   \\ \hline
\end{tabular}
\end{table}








\subsection{Varying the speed of light $c$}
In order to focus on the role of the speed of light $c$, we computed the ESS of the chains obtained by running RHMC at each point of grid of values of $\epsilon \times c$ and $\epsilon$. Figure \ref{fig:gmm_contour} shows the contour plot of the ESS for the Gaussian mixture model with $\sigma^2 = 1$. The ESS was %computed at 20 equally spaced values between 0.01 and 4 of $\epsilon \times c$ and 40 equally spaced values of stepsize $\epsilon$ between 0.01 and 8 and 
averaged over 100 chains of length $1 \times 10^5$. The optimal ESS represented by the red dot corresponds to $c = 0.63$ and $\epsilon = 3.90$, resulting in $\epsilon \times c = 2.457$. The quantity $\epsilon \times c$ can be thought of as the maximum length scale of the updates. The idea is that the speed of light $c$ allows to choose the desired maximum length scale and can be tuned according to the target distribution at hand. Figure \ref{fig:gmm_mass} shows the relationship between $m$ and some quantities of interest at the values of $c$ and $\epsilon$ optimizing the ESS. %The plots were obtained by averaging the three quantities over 300 chains of length 10000 at each of 1000 equally spaced mass values between 0.001 and 10.0. 
Observe the different roles of $c$ and $m$: while the speed of light $c$ controls the maximum speed of the particles, the mass parameter $m$ controls their average speed.


\begin{figure*}[]
\centering
\includegraphics[width=0.6\textwidth]{plots_GMM/gmm_contour} 
\caption {Contour plot of the ESS. The product $\epsilon \times c$ represents the maximum length scale of the updates in RHMC.}
\label{fig:gmm_contour}
\end{figure*}

\begin{figure*}[]
\centering
\includegraphics[width=0.8\textwidth]{plots_GMM/gmm_mass} 
\caption {Average speed, ESS and acceptance rate at the stepsize maximizing the ESS. The red horizontal line corresponds to the speed of light $c$.}
\label{fig:gmm_mass}
\end{figure*}



==> experiments.tex <==
\section{Experiments}


\subsection{Gaussian mixture models}
Consider a simple univariate model obtained by combining the three following Gaussian random variables with equal mixing proportions: $ \mathcal{N}(-5,1/ \sigma^2)$,  $\mathcal{N}(0,\sigma^2)$,  $\mathcal{N}(5,1/\sigma^2)$. We picked the value of $\sigma^2$ from the set $\{1,0.5,0.3 \}$, giving rise to three different Gaussian mixture models (see the top row of Figure \ref{gmm_MAE_STEIN}). Note that when $\sigma^2=1$ the three Gaussians have the same variance while, the lower $\sigma^2$, the larger the discrepancy between their variances and thus the wider the range of values taken by the gradient of the target density. We compare the performance of HMC and RHMC for a wide range of stepsize values. The goal is to verify whether the relativistic dynamics is more robust to the choice of the stepsize and allows for a more efficient exploration of the target density.  


Figure \ref{gmm_MAE_STEIN} shows the mean absolute error (MAE) and the log of the Stein discrepancy as a function of the stepsize for each of the three Gaussian mixture models. The MAE is computed as the L1 distance between the sample frequencies and the true probabilities, obtained by partitioning the interval [-10,10] with 100 bins of size 0.2. The Stein discrepancy is an additional way to quantify the maximum discrepancy between sample and target expectations [see Measuring Sample Quality with Stein's Method]. The MAE and Stein discrepancy were averaged over 100 different chains each with $1 \times 10^6$ samples at 80 equally spaced stepsizes from 0.1 to 8.0. In the examples is these section, we set the mass parameter $m=1$ and the number of leapfrog steps to 10. As expected, RHMC is strikingly more robust to the stepsize compared to HMC, which fails to explore the target distribution and results in large MAE and log stein discrepancy, especially when the stepsize is large. Moreover, when the gradients of the target model span a large range of values, the improvements yielded by the relativistic dynamics are more pronounced. These results confirm that, since the speed of particles is bounded by $c$, RHMC is less sensitive to the presence of peaked gradients in the target density and more stable with respect to the choice of the stepsize. 


We then compared the efficiency of HMC and RHMC in exploring the target density by analyzing the ESS and acceptance rate of the Markov chains. Consistently with the previous results, RHMC is more stable to the choice of the stepsize and allows to reach greater ESS values.

Finally, we picked the optimal step sizes minimising the MAE error and compared the ESS between HMC and RHMC. The ESS values at the optimal stepsize is shown in Table \ref{table:ESS}, where we report the mean and one standard deviation after running 100 different chains of $1 \times 10^6$ samples each. First, RHMC exhibits a significantly more efficient convergence at these optimal step sizes. Second, when the gradient of the target density spans a wide range of values, as it is the case with Model 3, the improvement in efficiency yielded by the relativistic dynamics is even more pronounced. 


\begin{figure*}[]  
\centering
\includegraphics[width=1\textwidth]{plots_GMM/gmm_MAE_STEIN} 
\caption {Mean absolute error (MAE) and log of the Stein discrepancy against stepsize for three different Gaussian mixture models. }
\label{fig:bins}
\label{gmm_MAE_STEIN}
\end{figure*}



\begin{figure*}[]
\centering
\includegraphics[width=1\textwidth]{plots_GMM/gmm_ESS_ACC} 
\caption {Effective sample size (ESS) and acceptance rate against stepsize for three different Gaussian mixture models.}
\label{fig:bins}
\end{figure*}




\begin{table}[]
\centering
\caption{Comparison between the ESS for RHMC and HMC given the optimal stepsize minimizing the MAE. The table shows the mean and one standard deviation over 100 different runs. RHMC consistently outperforms HMC and the improvement is more pronounced in Model 3, where the gradient of the target model spans a large range of values.}
\label{table:ESS}
\begin{tabular}{|l|l|l|l|l|}
\hline
ESS  & Model 1 & Model 2 & Model 3 \\ \hline
RHMC &\textbf{70119.5}  $\pm$ \textbf{875.3}  & \textbf{47785.0} $\pm$ \textbf{848.0} & \textbf{109659.9}  $\pm$ \textbf{1408.8}   \\ \hline

HMC &35970.8  $\pm$ 558.5 &29659.6  $\pm$   577.1  &  20675.4 $\pm$ 558.5   \\ \hline
\end{tabular}
\end{table}








\subsubsection{Varying the speed of light $c$}
In order to focus on the role of the speed of light $c$, we considered the performance of RHMC in terms of ESS at each point of grid of values of $\epsilon \times c$ and $\epsilon$. Figure \ref{fig:gmm_contour} shows the contour plot of the ESS for the Gaussian mixture model with $\sigma^2 = 1$. The ESS was computed at 20 equally spaced values between 0.01 and 4 of $\epsilon \times c$ and 40 equally spaced values of stepsize $\epsilon$ between 0.01 and 8 and averaged over 100 chains of length $1 \times 10^5$. The optimal ESS represented by the red dot corresponds to $c = 0.63$ and $\epsilon = 3.90$, resulting in a length scale $\epsilon \times c$ equal to $2.457$. The quantity $\epsilon \times c$ on the $y$-axis can be thought of as the maximum length scale of the updates in RHMC. The idea is that the speed of light $c$ allows to choose the desired maximum length scale and can be tuned according to the target distribution at hand. 

Finally, given the values of $c$ and $\epsilon$ optimizing the ESS, we show the relationship between $m$ and the average speed of the particles, the ESS and the acceptance rate in Figure \ref{fig:gmm_mass}. %The plots were obtained by averaging the three quantities over 300 chains of length 10000 at each of 1000 equally spaced mass values between 0.001 and 10.0. 
Observe that, while the speed of light $c$ controls the maximum speed of the particles, the mass parameter $m$ controls their average speed.


\begin{figure*}[]
\centering
\includegraphics[width=0.6\textwidth]{plots_GMM/gmm_contour} 
\caption {Contour plot of the ESS. The product $\epsilon \times c$ represents the maximum length scale of the updates in RHMC.}
\label{fig:gmm_contour}
\end{figure*}

\begin{figure*}[]
\centering
\includegraphics[width=0.8\textwidth]{plots_GMM/gmm_mass} 
\caption {Average speed, ESS and acceptance rate at the stepsize maximizing the ESS. The red horizontal line corresponds to the speed of light $c$.}
\label{fig:gmm_mass}
\end{figure*}

